Learning Blind Video Temporal Consistency

Applying image processing algorithms independently to each frame of a video often leads to undesired inconsistent results over time. Developing temporally consistent video-based extensions, however, requires domain knowledge for individual tasks and is unable to generalize to other applications. In this paper, we present an efficient end-to-end approach based on deep recurrent network for enforcing temporal consistency in a video. Our method takes the original unprocessed and per-frame processed videos as inputs to produce a temporally consistent video. Consequently, our approach is agnostic to specific image processing algorithms applied on the original video. We train the proposed network by minimizing both short-term and long-term temporal losses as well as the perceptual loss to strike a balance between temporal stability and perceptual similarity with the processed frames. At test time, our model does not require computing optical flow and thus achieves real-time speed even for high-resolution videos. We show that our single model can handle multiple and unseen tasks, including but not limited to artistic style transfer, enhancement, colorization, image-to-image translation and intrinsic image decomposition. Extensive objective evaluation and subject study demonstrate that the proposed approach performs favorably against the state-of-the-art methods on various types of videos.

==> tables/analysis.tex <==
%MH: figures are not aligned well.
\begin{figure}[t]
    \centering
    \scriptsize
    \begin{minipage}[b]{0.47\textwidth}
        \centering
        \begin{tabular}{C{0.8cm}C{0.8cm}C{0.9cm}|C{1.4cm}C{1.4cm}}
            \toprule
            $\lambda_t$ & $\lambda_p$ & $r= \frac{\lambda_t}{\lambda_p}$ &
            $E_{\text{warp}}$ & $D_{\text{perceptual}}$
            \\
            \midrule
            10    &  0.01  &  1000  &  0.0279 & 0.1744 \\
            10    &  0.1   &  100   &  0.0265 & 0.1354 \\
            10    &  1     &  10    &  0.0615 & 0.0071 \\
            10    &  10    &  1     &  0.0621 & 0.0072 \\
            100   &  1     &  100   &  0.0277 & 0.1324 \\
            100   &  10    &  10    &  \red{0.0442} & \red{0.0170} \\
            100   &  100   &  1     &  0.0621 & 0.0072 \\
            1000  &  1     &  1000  &  0.0262 & 0.1848 \\
            1000  &  10    &  100   &  0.0275 & 0.1341 \\
            1000  &  100   &  10    &  \red{0.0453} & \red{0.0158} \\
            1000  &  1000  &  1     &  0.0621 & 0.0072 \\
            \bottomrule
        \end{tabular}
        \label{tab:trade_off}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.47\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{trade_off/curve_v2_font.pdf} 
    \end{minipage}
    \vspace{-1mm}
    \caption{
        \textbf{Analysis of parameters}.
        (Left) When $\lambda_t$ is large enough, choosing $r = 10$ (shown in red) achieves a good balance between reducing temporal warping error as well as perceptual distance.
        (Right) The trade off between perceptual similarity and temporal warping with different ratios $r$, as compared to Bonneel et al.~\protect\cite{Bonneel-TOG-2015}, and the original processed video, $V_p$.
    }
    \label{fig:trade_off}
    \vspace{-2mm}
\end{figure}


==> tables/blind_comparison.tex <==

\begin{table}[t]
	\centering
	\scriptsize
	\caption{
		\textbf{Comparison of blind temporal consistency methods}.
		%
		Both the methods of Bonneel~\etal~\cite{Bonneel-TOG-2015} and Yao~\etal~\cite{Yao-MM-2017} require dense correspondences from optical flow or PatchMatch~\cite{PatchMatch}, while the proposed method does not explicitly rely on these correspondences at test time. 
		%only needs the input and processed frames to generate the results.
		%
		The algorithm of Yao~\etal~\cite{Yao-MM-2017} involves a key-frame selection from the entire video and thus cannot generate output in an online manner.
	}
	\begin{tabular}{c|C{2.5cm}C{2.5cm}C{2.5cm}}
		\toprule
		& Bonneel~\etal~\cite{Bonneel-TOG-2015} & Yao~\etal~\cite{Yao-MM-2017} & Ours
		\\
		\midrule
		Content constraint &
		gradient & local affine & perceptual loss \\
		Short-term temporal constraint &
		\checkmark & - & \checkmark \\
		Long-term temporal constraint &
		- & \checkmark & \checkmark \\
		Require dense correspondences & 
		\multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{-} \\
		(at test time) & & & \\
		Online processing &
		\checkmark & - & \checkmark \\
		\bottomrule
	\end{tabular}
	\vspace{-2mm}
	\label{tab:blind_comparison}
\end{table}

==> tables/perceptual.tex <==
\begin{table}
	\centering
	\scriptsize
	\caption{
		\textbf{Quantitative evaluation on perceptual distance}.
		%
		Our method has lower perceptual distance than Bonneel~\etal~\cite{Bonneel-TOG-2015}.
	}
	\vspace{1mm}
	\begin{tabular}{l|c|C{1cm}C{1cm}|C{1cm}C{1cm}}
		\toprule
		\multirow{2}{*}{Task} &
		\multirow{2}{*}{Trained} &
		\multicolumn{2}{c|}{\textsc{Davis}} &
		\multicolumn{2}{c}{\textsc{Videvo}} \\
		& 
		& \cite{Bonneel-TOG-2015} 
		& Ours 
		& \cite{Bonneel-TOG-2015} 
		& Ours 
		\\
		\midrule
		WCT~\cite{WCT}/antimono & \checkmark &
		0.098 & \textbf{0.019} & 0.106 & \textbf{0.016}
		\\
		WCT~\cite{WCT}/asheville &  &
		0.090 & \textbf{0.019} & 0.098 & \textbf{0.015}
		\\
		WCT~\cite{WCT}/candy & \checkmark &
		0.133 & \textbf{0.023} & 0.139 & \textbf{0.018}
		\\
		WCT~\cite{WCT}/feathers & &
		0.093 & \textbf{0.016} & 0.100 & \textbf{0.011}
		\\
		WCT~\cite{WCT}/sketch & \checkmark &
		0.042 & \textbf{0.021} & 0.046 & \textbf{0.014}
		\\
		WCT~\cite{WCT}/wave & &
		0.065 & \textbf{0.015} & 0.072 & \textbf{0.013}
		\\
		Fast-neural-style~\cite{Johnson-ECCV-2016}/princess &  &
		0.143 & \textbf{0.029} & 0.165 & \textbf{0.018}
		\\
		Fast-neural-style~\cite{Johnson-ECCV-2016}/udnie &  &
		0.070 & \textbf{0.017} & 0.076 & \textbf{0.014}
		\\
		DBL~\cite{DBL}/expertA & \checkmark &
		0.026 & \textbf{0.011} & 0.033 & \textbf{0.007}
		\\
		DBL~\cite{DBL}/expertB & &
		0.023 & \textbf{0.011} & 0.030 & \textbf{0.007}
		\\
		Intrinsic~\cite{Bell-TOG-2014}/reflectance &  &
		0.044 & \textbf{0.013} & 0.056 & \textbf{0.008}
		\\
		Intrinsic~\cite{Bell-TOG-2014}/shading & \checkmark &
		0.029 & \textbf{0.017} & 0.032 & \textbf{0.009}
		\\
		CycleGAN~\cite{CycleGAN}/photo2ukiyoe &  &
		0.042 & \textbf{0.012} & 0.054 & \textbf{0.007}
		\\
		CycleGAN~\cite{CycleGAN}/photo2vangogh &  &
		0.067 & \textbf{0.016} & 0.079 & \textbf{0.011}
		\\
		Colorization~\cite{Zhang-ECCV-2016} & \checkmark &
		0.062 & \textbf{0.013} & 0.055 & \textbf{0.009}
		\\
		Colorization~\cite{Iizuka-TOG-2016} & &
		0.033 & \textbf{0.011} & 0.034 & \textbf{0.008}
		\\
		\midrule
		Average & &
		0.088 & \textbf{0.017} & 0.073 & \textbf{0.012}
		\\
		\bottomrule
	\end{tabular}
	\label{tab:perceptual}
	\vspace{-1mm}
\end{table}

==> tables/warp_error.tex <==
\begin{table}[t]
	\centering
	\scriptsize
	\caption{
		\textbf{Quantitative evaluation on temporal warping error}.
		%
		The ``Trained'' column indicates the applications used for training our model.
		%
		Our method achieves a similarly reduced temporal warping error as Bonneel~\etal~\cite{Bonneel-TOG-2015}, which is significantly less than the original processed video ($V_p$). 
		%\ow{define ``Trained''. Should there be an average column? Because it looks like [14] is maybe lower than ours, but maybe the average will show we are lower, if so we can add this.}
	}
	\vspace{1mm}
	\begin{tabular}{l|c|C{1cm}C{1cm}C{1cm}|C{1cm}C{1cm}C{1cm}}
		\toprule
		\multirow{2}{*}{Task} &
		\multirow{2}{*}{Trained} &
		\multicolumn{3}{c|}{\textsc{Davis}} &
		\multicolumn{3}{c}{\textsc{Videvo}} \\
		& & $V_p$
		& \cite{Bonneel-TOG-2015} 
		& Ours 
		& $V_p$
		& \cite{Bonneel-TOG-2015} 
		& Ours 
		\\
		\midrule
		WCT~\cite{WCT}/antimono & \checkmark &
		0.054 & \textbf{0.031} & 0.035 & 0.025 & 0.014 & \textbf{0.013}
		\\
		WCT~\cite{WCT}/asheville & &
		0.088 & \textbf{0.047} & 0.055 & 0.045 & 0.025 & \textbf{0.023}
		\\
		WCT~\cite{WCT}/candy & \checkmark &
		0.069 & \textbf{0.037} & 0.045 & 0.034 & \textbf{0.018} & \textbf{0.018}
		\\
		WCT~\cite{WCT}/feathers & &
		0.052 & \textbf{0.029} & \textbf{0.029} & 0.027 & 0.016 & \textbf{0.012}
		\\
		WCT~\cite{WCT}/sketch & \checkmark &
		0.046 & 0.028 & \textbf{0.023} & 0.022 & 0.015 & \textbf{0.009}
		\\
		WCT~\cite{WCT}/wave & &
		0.049 & 0.030 & \textbf{0.027} & 0.026 & 0.015 & \textbf{0.011}
		\\
		Fast-neural-style~\cite{Johnson-ECCV-2016}/princess &  &
		0.073 & 0.048 & \textbf{0.047} & 0.039 & 0.023 & \textbf{0.021}
		\\
		Fast-neural-style~\cite{Johnson-ECCV-2016}/udnie &  &
		0.065 & \textbf{0.039} & 0.042 & 0.028 & 0.017 & \textbf{0.015}
		\\
		DBL~\cite{DBL}/expertA & \checkmark &
		0.039 & 0.035 & \textbf{0.028} & 0.018 & 0.016 & \textbf{0.010}
		\\
		DBL~\cite{DBL}/expertB & &
		0.034 & 0.031 & \textbf{0.025} & 0.015 & 0.014 & \textbf{0.008}
		\\
		Intrinsic~\cite{Bell-TOG-2014}/reflectance &  &
		0.024 & 0.020 & \textbf{0.015} & 0.012 & 0.008 & \textbf{0.005}
		\\
		Intrinsic~\cite{Bell-TOG-2014}/shading & \checkmark &
		0.016 & 0.012 & \textbf{0.009} & 0.008 & 0.006 & \textbf{0.003}
		\\
		CycleGAN~\cite{CycleGAN}/photo2ukiyoe &  &
		0.037 & 0.030 & \textbf{0.026} & 0.019 & 0.016 & \textbf{0.010}
		\\
		CycleGAN~\cite{CycleGAN}/photo2vangogh &  &
		0.040 & 0.032 & \textbf{0.029} & 0.021 & 0.017 & \textbf{0.013}
		\\
		Colorization~\cite{Zhang-ECCV-2016} & \checkmark &
		0.030 & 0.028 & \textbf{0.024} & 0.012 & 0.011 & \textbf{0.008}
		\\
		Colorization~\cite{Iizuka-TOG-2016} & &
		0.030 & 0.028 & \textbf{0.023} & 0.012 & 0.011 & \textbf{0.008}
		\\
		\midrule
		Average & &
		0.047 & 0.032 & \textbf{0.030} & 0.023 & 0.015 & \textbf{0.012}
		\\
		\bottomrule
	\end{tabular}
	\label{tab:warp_error}
	\vspace{-2mm}
\end{table}
